How Much Can Time-related Features Enhance Time Series Forecasting?

Recent advancements in long-term time series forecasting (LTSF) have primarily focused on capturing cross-time and cross-variate (channel) dependencies within historical data. However, a critical aspect often overlooked by many existing methods is the explicit incorporation of \textbf{time-related features} (e.g., season, month, day of the week, hour, minute), which are essential components of time series data. The absence of this explicit time-related encoding limits the ability of current models to capture cyclical or seasonal trends and long-term dependencies, especially with limited historical input. To address this gap, we introduce a simple yet highly efficient module designed to encode time-related features, Time Stamp Forecaster (TimeSter), thereby enhancing the backbone's forecasting performance. By integrating TimeSter with a linear backbone, our model, TimeLinear, significantly improves the performance of a single linear projector, reducing MSE by an average of 23\% on benchmark datasets such as Electricity and Traffic. Notably, TimeLinear achieves these gains while maintaining exceptional computational efficiency, delivering results that are on par with or exceed state-of-the-art models, despite using a fraction of the parameters.

==> table/ablation_time_feature.tex <==
\begin{table}[htpb]
\caption{Ablation Time Features Hour}
\centering
\label{tab:ablation_timefeatures_hour}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|cccccccc}

\toprule[1pt]
\multirow{2}{*}{Time Features} & \multicolumn{2}{c}{ETTh1} & \multicolumn{2}{c}{ETTh2} & \multicolumn{2}{c}{Electricity} & \multicolumn{2}{c}{Traffic} \\
\cmidrule(l{10pt}r{10pt}){2-3}\cmidrule(l{10pt}r{10pt}){4-5}\cmidrule(l{10pt}r{10pt}){6-7}\cmidrule(l{10pt}r{10pt}){8-9}
& MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\toprule[1pt]

- &  &  &  \\
\midrule

Hour &  &  &  \\
\midrule

Hour\_Day &  &  &  \\
\midrule

Hour\_Month &  &  &  \\
\midrule

Hour\_Season &  &  &  \\
\midrule

Hour\_Day\_Month &  &  &  \\
\midrule

Hour\_Day\_Season  &  &  &  \\
\midrule

Hour\_Month\_Season  &  &  &  \\
\midrule

Hour\_Day\_Month\_Season  &  & \textbf{\textcolor{red}{}} & \textbf{\textcolor{red}{}} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table}

\begin{table}[htpb]
\caption{Ablation Time Features Minute}
\centering
\label{tab:ablation_timefeatures_min}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|cccccc}

\toprule[1pt]
\multirow{2}{*}{Time Features} & \multicolumn{2}{c}{ETTm1} & \multicolumn{2}{c}{ETTm2} & \multicolumn{2}{c}{Weather} \\
\cmidrule(l{10pt}r{10pt}){2-3}\cmidrule(l{10pt}r{10pt}){4-5}\cmidrule(l{10pt}r{10pt}){6-7}
& MSE & MAE & MSE & MAE & MSE & MAE \\
\toprule[1pt]

- &  &  &  \\
\midrule

Minute\_Hour &  &  &  \\
\midrule

Minute\_Hour\_Day &  &  &  \\
\midrule

Minute\_Hour\_Month &  &  &  \\
\midrule

Minute\_Hour\_Season &  &  &  \\
\midrule

Minute\_Hour\_Day\_Month &  &  &  \\
\midrule

Minute\_Hour\_Day\_Season  &  &  &  \\
\midrule

Minute\_Hour\_Month\_Season  &  &  &  \\
\midrule

Minute\_Hour\_Day\_Month\_Season  &  & \textbf{\textcolor{red}{}} & \textbf{\textcolor{red}{}} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table}


==> table/ablation_time_feature_old.tex <==
\begin{table}[htpb]
\caption{Ablation Time Features}
\centering
\label{tab:ablation_timefeatures_hour}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccc|cccc}

\toprule[1pt]
Hour & Day & Month & Season & ETTh1 & ETTh2 & Electricity & Traffic \\
\toprule[1pt]

\checkmark & - & - & - &  &  &  \\
\midrule

\checkmark & \checkmark & - & - &  &  &  \\
\midrule

\checkmark & - & \checkmark & - &  &  &  \\
\midrule

\checkmark & - & - & \checkmark &  &  &  \\
\midrule

\checkmark & \checkmark & \checkmark & - &  &  &  \\
\midrule

\checkmark & \checkmark & - & \checkmark &  &  &  \\
\midrule

\checkmark & - & \checkmark & \checkmark &  &  &  \\
\midrule

\checkmark & \checkmark & \checkmark & \checkmark &  & \textbf{\textcolor{red}{}} & \textbf{\textcolor{red}{}} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table}

\begin{table}[htpb]
\caption{Ablation Time Features}
\centering
\label{tab:ablation_timefeatures_min}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccc|ccc}

\toprule[1pt]
Minute & Hour & Day & Month & Season & ETTm1 & ETTm2 & Weather \\
\toprule[1pt]

\checkmark & \checkmark & - & - & - &  &  &  \\
\midrule

\checkmark & \checkmark & \checkmark & - & - &  &  &  \\
\midrule

\checkmark & \checkmark & - & \checkmark & - &  &  &  \\
\midrule

\checkmark & \checkmark & - & - & \checkmark &  &  &  \\
\midrule

\checkmark & \checkmark & \checkmark & \checkmark & - &  &  &  \\
\midrule

\checkmark & \checkmark & \checkmark & - & \checkmark &  &  &  \\
\midrule

\checkmark & \checkmark & - & \checkmark & \checkmark &  &  &  \\
\midrule

\checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  & \textbf{\textcolor{red}{}} & \textbf{\textcolor{red}{}} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table}









\begin{table}[htpb]
\caption{Ablation Time Features}
\centering
\label{tab:ablation_timefeatures_hour}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|cccccccc}

\toprule[1pt]
\multirow{2}{*}{Time Features} & \multicolumn{2}{c}{ETTh1} & \multicolumn{2}{c}{ETTh2} & \multicolumn{2}{c}{Electricity} & \multicolumn{2}{c}{Traffic} \\
\cmidrule(l{10pt}r{10pt}){2-3}\cmidrule(l{10pt}r{10pt}){4-5}\cmidrule(l{10pt}r{10pt}){6-7}\cmidrule(l{10pt}r{10pt}){8-9}
& MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\toprule[1pt]

Hour &  &  &  \\
\midrule

Hour\_Day &  &  &  \\
\midrule

Hour\_Month &  &  &  \\
\midrule

Hour\_Season &  &  &  \\
\midrule

Hour\_Day\_Month &  &  &  \\
\midrule

Hour\_Day\_Season  &  &  &  \\
\midrule

Hour\_Month\_Month  &  &  &  \\
\midrule

Hour\_Day\_Month\_Season  &  & \textbf{\textcolor{red}{}} & \textbf{\textcolor{red}{}} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table}

\begin{table}[htpb]
\caption{Ablation Time Features}
\centering
\label{tab:ablation_timefeatures_min}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|cccccc}

\toprule[1pt]
\multirow{2}{*}{Time Features} & \multicolumn{2}{c}{ETTm1} & \multicolumn{2}{c}{ETTm2} & \multicolumn{2}{c}{Weather} \\
\cmidrule(l{10pt}r{10pt}){2-3}\cmidrule(l{10pt}r{10pt}){4-5}\cmidrule(l{10pt}r{10pt}){6-7}
& MSE & MAE & MSE & MAE & MSE & MAE \\
\toprule[1pt]

Minute\_Hour &  &  &  \\
\midrule

Minute\_Hour\_Day &  &  &  \\
\midrule

Minute\_Hour\_Month &  &  &  \\
\midrule

Minute\_Hour\_Season &  &  &  \\
\midrule

Minute\_Hour\_Day\_Month &  &  &  \\
\midrule

Minute\_Hour\_Day\_Season  &  &  &  \\
\midrule

Minute\_Hour\_Month\_Month  &  &  &  \\
\midrule

Minute\_Hour\_Day\_Month\_Season  &  & \textbf{\textcolor{red}{}} & \textbf{\textcolor{red}{}} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table}


==> table/generalization.tex <==
\begin{table*}[htpb]
\caption{Performance gain after combining TimeSter with other backbones.
The look-back window is $L=96$.
The average performance of four prediction lengths $T\in\{96,192,336,720\}$ are reported.
\textcolor{red}{Red} denotes improved performance and \textcolor[HTML]{5CAA82}{Green} indicates decreasing performance.
\textit{Model Promotion} denotes the average improvement of a model on all datasets.
\textit{Dataset Promotion} denotes the average improvement on a dataset of all models.
}
\centering
\label{tab:generalization}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{p{0.2cm}|c|cc|cc|cc|cc|cc|cc|cc|cc}

\toprule[1pt]
\multicolumn{2}{c}{Dataset} &
\multicolumn{2}{c}{ETTm1}  & \multicolumn{2}{c}{ETTm2} & \multicolumn{2}{c}{ETTh1} & \multicolumn{2}{c}{ETTh2} & \multicolumn{2}{c}{Electricity} & \multicolumn{2}{c}{Weather} & \multicolumn{2}{c}{Traffic} & \multicolumn{2}{c}{Model Promotion}  \\
\cmidrule(l{10pt}r{10pt}){1-2}\cmidrule(l{10pt}r{10pt}){3-4}\cmidrule(l{10pt}r{10pt}){5-6}\cmidrule(l{10pt}r{10pt}){7-8}\cmidrule(l{10pt}r{10pt}){9-10}\cmidrule(l{10pt}r{10pt}){11-12}\cmidrule(l{10pt}r{10pt}){13-14}\cmidrule(l{10pt}r{10pt}){15-16}\cmidrule(l{10pt}r{10pt}){17-18}
\multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\toprule[1pt]

\multirow{6}{*}{\rotatebox[origin=c]{90}{Linear}} & RLinear & 0.412 & 0.406 & 0.286 & 0.327 & 0.446 & 0.433 & 0.377 & 0.399 & 0.215 & 0.291 & 0.273 & 0.291 & 0.623 & 0.371 & \textcolor{red}{\multirow{3}{*}{10.47\%}} & \textcolor{red}{\multirow{3}{*}{6.40\%}} \\

& w / TimeSter & 0.385 & 0.395 & 0.273 & 0.315 & 0.432 & 0.426 & 0.358 & 0.389 & 0.165 & 0.259 & 0.251 & 0.276 & 0.480 & 0.304 \\

& Promotion & \textcolor{red}{6.43\%} & \textcolor{red}{2.64\%} & \textcolor{red}{4.68\%} & \textcolor{red}{3.67\%} & \textcolor{red}{3.11\%} & \textcolor{red}{1.64\%} & \textcolor{red}{5.02\%} & \textcolor{red}{2.64\%} & \textcolor{red}{23.04\%} & \textcolor{red}{11.06\%} & \textcolor{red}{8.02\%} & \textcolor{red}{5.10\%} & \textcolor{red}{22.96\%} & \textcolor{red}{18.07\%} \\
\cmidrule(l{10pt}r{10pt}){2-18}
& FITS & 0.415 & 0.408 & 0.286 & 0.328 & 0.444 & 0.432 & 0.374 & 0.397 & 0.217 & 0.295 & 0.273 & 0.292 & 0.627 & 0.375 & \textcolor{red}{\multirow{3}{*}{10.02\%}} & \textcolor{red}{\multirow{3}{*}{5.93\%}} \\

& w / TimeSter & 0.387 & 0.397 & 0.273 & 0.316 & 0.432 & 0.425 & 0.363 & 0.393 & 0.167 & 0.262 & 0.251 & 0.277 & 0.488 & 0.316 \\

& Promotion & \textcolor{red}{6.59\%} & \textcolor{red}{2.74\%} & \textcolor{red}{4.69\%} & \textcolor{red}{3.85\%} & \textcolor{red}{2.83\%} & \textcolor{red}{1.42\%} & \textcolor{red}{2.94\%} & \textcolor{red}{1.21\%} & \textcolor{red}{23.09\%} & \textcolor{red}{11.27\%} & \textcolor{red}{7.91\%} & \textcolor{red}{5.20\%} & \textcolor{red}{22.12\%} & \textcolor{red}{15.82\%} \\

\midrule

\multirow{6}{*}{\rotatebox[origin=c]{90}{Convolution}} & ModernTCN & 0.386 & 0.401 & 0.278 & 0.322 & 0.445 & 0.432 & 0.381 & 0.404 & 0.197 & 0.282 & 0.240 & 0.271 & 0.550 & 0.369 & \textcolor{red}{\multirow{3}{*}{4.13\%}} & \textcolor{red}{\multirow{3}{*}{3.30\%}} \\

& w / TimeSter & 0.382 & 0.399 & 0.275 & 0.319 & 0.444 & 0.432 & 0.377 & 0.401 & 0.171 & 0.265 & 0.237 & 0.267 & 0.492 & 0.321 \\

& Promotion & \textcolor{red}{1.05\%} & \textcolor{red}{0.56\%} & \textcolor{red}{1.09\%} & \textcolor{red}{0.87\%} & \textcolor{red}{0.23\%} & \textcolor{red}{0.22\%} & \textcolor{red}{1.18\%} & \textcolor{red}{0.75\%} & \textcolor{red}{13.33\%} & \textcolor{red}{5.90\%} & \textcolor{red}{1.37\%} & \textcolor{red}{1.67\%} & \textcolor{red}{10.63\%} & \textcolor{red}{13.12\%} \\
\cmidrule(l{10pt}r{10pt}){2-18}
& TimesNet & 0.408 & 0.415 & 0.295 & 0.332 & 0.473 & 0.463 & 0.407 & 0.421 & 0.195 & 0.295 & 0.261 & 0.287 & 0.624 & 0.331 & \textcolor{red}{\multirow{3}{*}{1.62\%}} & \textcolor{red}{\multirow{3}{*}{1.02\%}} \\

& w / TimeSter & 0.402 & 0.411 & 0.292 & 0.329 & 0.465 & 0.459 & 0.399 & 0.417 & 0.193 & 0.293 & 0.252 & 0.281 & 0.624 & 0.331 \\

& Promotion & \textcolor{red}{1.45\%} & \textcolor{red}{0.84\%} & \textcolor{red}{1.08\%} & \textcolor{red}{0.85\%} & \textcolor{red}{1.66\%} & \textcolor{red}{0.70\%} & \textcolor{red}{1.99\%} & \textcolor{red}{0.92\%} & \textcolor{red}{1.19\%} & \textcolor{red}{0.80\%} & \textcolor{red}{3.35\%} & \textcolor{red}{2.30\%} & \textcolor{red}{0.60\%} & \textcolor{red}{0.73\%} \\

\midrule

\multirow{6}{*}{\rotatebox[origin=c]{90}{Transformer}} & iTransformer & 0.408 & 0.412 & 0.291 & 0.335 & 0.458 & 0.449 & 0.383 & 0.407 & 0.178 & 0.269 & 0.260 & 0.280 & 0.422 & 0.282 & \textcolor{red}{\multirow{3}{*}{3.81\%}} & \textcolor{red}{\multirow{3}{*}{2.03\%}} \\

& w / TimeSter & 0.391 & 0.404 & 0.280 & 0.325 & 0.439 & 0.437 & 0.379 & 0.404 & 0.162 & 0.259 & 0.249 & 0.274 & 0.422 & 0.281 \\

& Promotion & \textcolor{red}{4.24\%} & \textcolor{red}{1.87\%} & \textcolor{red}{3.50\%} & \textcolor{red}{3.06\%} & \textcolor{red}{4.12\%} & \textcolor{red}{2.61\%} & \textcolor{red}{1.35\%} & \textcolor{red}{0.69\%} & \textcolor{red}{8.96\%} & \textcolor{red}{3.36\%} & \textcolor{red}{4.33\%} & \textcolor{red}{2.15\%} & \textcolor{red}{0.13\%} & \textcolor{red}{0.48\%} \\
\cmidrule(l{10pt}r{10pt}){2-18}

& PatchTST & 0.387 & 0.400 & 0.283 & 0.327 & 0.445 & 0.441 & 0.378 & 0.403 & 0.191 & 0.280 & 0.256 & 0.278 & 0.461 & 0.291 & \textcolor{red}{\multirow{3}{*}{4.02\%}} & \textcolor{red}{\multirow{3}{*}{1.26\%}} \\

& w / TimeSter & 0.379 & 0.401 & 0.278 & 0.324 & 0.438 & 0.439 & 0.374 & 0.402 & 0.170 & 0.268 & 0.244 & 0.272 & 0.442 & 0.291 \\

& Promotion & \textcolor{red}{2.15\%} & \textcolor[HTML]{5CAA82}{-0.18\%} & \textcolor{red}{2.02\%} & \textcolor{red}{0.95\%} & \textcolor{red}{1.57\%} & \textcolor{red}{0.44\%} & \textcolor{red}{1.85\%} & \textcolor{red}{0.93\%} & \textcolor{red}{11.20\%} & \textcolor{red}{4.25\%} & \textcolor{red}{5.08\%} & \textcolor{red}{2.42\%} & \textcolor{red}{4.26\%} & \textcolor{red}{0.02\%} \\
\midrule

\multicolumn{2}{c|}{Dataset Promotion} & \textcolor{red}{3.65\%} & \textcolor{red}{1.41\%} & \textcolor{red}{2.84\%} & \textcolor{red}{2.21\%} & \textcolor{red}{2.25\%} & \textcolor{red}{1.17\%} & \textcolor{red}{2.39\%} & \textcolor{red}{1.19\%} & \textcolor{red}{13.47\%} & \textcolor{red}{6.11\%} & \textcolor{red}{5.01\%} & \textcolor{red}{3.14\%} & \textcolor{red}{10.12\%} & \textcolor{red}{8.04\%} \\

% Data goes here
\bottomrule[1pt]
\end{tabular}
}
% \vspace{-.18cm}
\end{table*}


==> table/generalization_full_old.tex <==
% \begin{table*}[htpb]
% \setcitestyle{round,numbers,comma}
% \caption{Full results of the long-term forecasting task. We fix the look-back window $L=96$ and make predictions for $T=\{96,192,336,720\}$. Avg means the average metrics for four prediction lengths. The best is highlighted in \textbf{\textcolor{red}{red}} and the runner-up in \underline{\textcolor{blue}{blue}}. We report the average results of three random seeds.}
% \centering
% \label{tab:generalization_full}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{p{0.2cm}c|cc|cc|cc|cc|cc|cc|cc|cc|cc}

% \toprule[1pt]

% \multicolumn{2}{c|}{Models} & \multicolumn{2}{c}{\makecell{RLinear\\\cite{li2023revisiting}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c|}{Promotion} & \multicolumn{2}{c}{\makecell{FITS\\\cite{xu2023fits}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c|}{Promotion} & \multicolumn{2}{c}{\makecell{ModernTCN\\\cite{luo2024moderntcn}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c}{Promotion} \\

% \cmidrule(l{10pt}r{10pt}){3-4}\cmidrule(l{10pt}r{10pt}){5-6}\cmidrule(l{10pt}r{10pt}){7-8}\cmidrule(l{10pt}r{10pt}){9-10}\cmidrule(l{10pt}r{10pt}){11-12}\cmidrule(l{10pt}r{10pt}){13-14}

% \multicolumn{2}{c|}{Metric} & MSE & MAE  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\

% \toprule[1pt]
% \multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm1}}
% & \multicolumn{1}{|c|}{96} & 0.350 & 0.370 & 0.325 & 0.364 & \textcolor{red}{7.06\%} & \textcolor{red}{1.78\%} & 0.353 & 0.374 & 0.329 & 0.368 & \textcolor{red}{6.77\%} & \textcolor{red}{1.73\%} & 0.317 & 0.362 & 0.315 & 0.359 & \textcolor{red}{0.59\%} & \textcolor{red}{0.64\%} \\

% & \multicolumn{1}{|c|}{192} & 0.389 & 0.390 & 0.365 & 0.381 & \textcolor{red}{6.13\%} & \textcolor{red}{2.26\%} & 0.392 & 0.393 & 0.366 & 0.383 & \textcolor{red}{6.55\%} & \textcolor{red}{2.49\%} & 0.317 & 0.362 & 0.315 & 0.359 & \textcolor{red}{1.62\%} & \textcolor{red}{0.55\%} \\

% & \multicolumn{1}{|c|}{336} & 0.422 & 0.413 & 0.395 & 0.401 & \textcolor{red}{6.43\%} & \textcolor{red}{2.88\%} & 0.425 & 0.415 & 0.397 & 0.402 & \textcolor{red}{6.67\%} & \textcolor{red}{2.98\%} & 0.403 & 0.412 & 0.399 & 0.411 & \textcolor{red}{1.03\%} & \textcolor{red}{0.06\%} \\

% & \multicolumn{1}{|c|}{720} & 0.486 & 0.448 & 0.456 & 0.433 & \textcolor{red}{6.23\%} & \textcolor{red}{3.47\%} & 0.488 & 0.450 & 0.457 & 0.434 & \textcolor{red}{6.42\%} & \textcolor{red}{3.57\%} & 0.461 & 0.443 & 0.457 & 0.439 & \textcolor{red}{0.94\%} & \textcolor{red}{0.96\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.412 & 0.406 & 0.385 & 0.395 & \textcolor{red}{6.43\%} & \textcolor{red}{2.64\%} & 0.415 & 0.408 & 0.387 & 0.397 & \textcolor{red}{6.59\%} & \textcolor{red}{2.74\%} & 0.386 & 0.401 & 0.382 & 0.399 & \textcolor{red}{1.05\%} & \textcolor{red}{0.56\%} \\

% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}
% & \multicolumn{1}{|c|}{96}& 0.183 & 0.264 & 0.167 & 0.249 & \textcolor{red}{8.48\%} & \textcolor{red}{5.97\%} & 0.183 & 0.266 & 0.168 & 0.249 & \textcolor{red}{8.54\%} & \textcolor{red}{6.25\%} & 0.173 & 0.255 & 0.169 & 0.252 & \textcolor{red}{1.85\%} & \textcolor{red}{1.14\%} \\

% & \multicolumn{1}{|c|}{192} & 0.246 & 0.304 & 0.233 & 0.291 & \textcolor{red}{5.41\%} & \textcolor{red}{4.28\%} & 0.248 & 0.305 & 0.234 & 0.292 & \textcolor{red}{5.45\%} & \textcolor{red}{4.44\%} & 0.235 & 0.296 & 0.237 & 0.297 & \textcolor[HTML]{5CAA82}{-0.88\%} & \textcolor[HTML]{5CAA82}{-0.20\%} \\

% & \multicolumn{1}{|c|}{336} & 0.307 & 0.342 & 0.295 & 0.331 & \textcolor{red}{4.11\%} & \textcolor{red}{3.24\%} & 0.308 & 0.343 & 0.295 & 0.332 & \textcolor{red}{4.14\%} & \textcolor{red}{3.34\%} & 0.308 & 0.344 & 0.299 & 0.336 & \textcolor{red}{2.80\%} & \textcolor{red}{2.20\%} \\

% & \multicolumn{1}{|c|}{720} & 0.407 & 0.398 & 0.395 & 0.390 & \textcolor{red}{2.96\%} & \textcolor{red}{2.03\%} & 0.408 & 0.398 & 0.396 & 0.390 & \textcolor{red}{2.92\%} & \textcolor{red}{2.25\%} & 0.398 & 0.394 & 0.395 & 0.392 & \textcolor{red}{0.61\%} & \textcolor{red}{0.34\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.286 & 0.327 & 0.273 & 0.315 & \textcolor{red}{4.68\%} & \textcolor{red}{3.67\%} & 0.286 & 0.328 & 0.273 & 0.316 & \textcolor{red}{4.69\%} & \textcolor{red}{3.85\%} & 0.278 & 0.322 & 0.275 & 0.319 & \textcolor{red}{1.09\%} & \textcolor{red}{0.87\%} \\

% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh1}}
% & \multicolumn{1}{|c|}{96}& 0.389 & 0.395 & 0.378 & 0.391 & \textcolor{red}{2.75\%} & \textcolor{red}{1.00\%} & 0.386 & 0.394 & 0.378 & 0.392 & \textcolor{red}{2.00\%} & \textcolor{red}{0.42\%} & 0.386 & 0.394 & 0.385 & 0.394 & \textcolor{red}{0.09\%} & \textcolor{red}{0.05\%} \\

% & \multicolumn{1}{|c|}{192} & 0.437 & 0.424 & 0.424 & 0.418 & \textcolor{red}{2.95\%} & \textcolor{red}{1.24\%} & 0.438 & 0.424 & 0.424 & 0.418 & \textcolor{red}{3.34\%} & \textcolor{red}{1.48\%} & 0.436 & 0.423 & 0.436 & 0.423 & \textcolor{red}{0.01\%} & \textcolor{red}{0.01\%} \\

% & \multicolumn{1}{|c|}{336} & 0.479 & 0.445 & 0.463 & 0.438 & \textcolor{red}{3.29\%} & \textcolor{red}{1.41\%} & 0.479 & 0.444 & 0.460 & 0.436 & \textcolor{red}{3.89\%} & \textcolor{red}{1.85\%} & 0.479 & 0.445 & 0.477 & 0.444 & \textcolor{red}{0.37\%} & \textcolor{red}{0.22\%} \\

% & \multicolumn{1}{|c|}{720} & 0.480 & 0.469 & 0.464 & 0.456 & \textcolor{red}{3.35\%} & \textcolor{red}{2.75\%} & 0.474 & 0.464 & 0.464 & 0.456 & \textcolor{red}{1.92\%} & \textcolor{red}{1.80\%} & 0.481 & 0.469 & 0.479 & 0.466 & \textcolor{red}{0.40\%} & \textcolor{red}{0.54\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.446 & 0.433 & 0.432 & 0.426 & \textcolor{red}{3.11\%} & \textcolor{red}{1.64\%} & 0.444 & 0.432 & 0.432 & 0.425 & \textcolor{red}{2.82\%} & \textcolor{red}{1.42\%} & 0.445 & 0.432 & 0.444 & 0.432 & \textcolor{red}{0.23\%} & \textcolor{red}{0.22\%} \\

% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}
% & \multicolumn{1}{|c|}{96}& 0.291 & 0.339 & 0.285 & 0.335 & \textcolor{red}{1.93\%} & \textcolor{red}{1.17\%} & 0.290 & 0.339 & 0.287 & 0.337 & \textcolor{red}{0.97\%} & \textcolor{red}{0.53\%} & 0.292 & 0.340 & 0.290 & 0.339 & \textcolor{red}{0.35\%} & \textcolor{red}{0.40\%} \\

% & \multicolumn{1}{|c|}{192} & 0.376 & 0.390 & 0.373 & 0.390 & \textcolor{red}{0.80\%} & \textcolor{red}{0.07\%} & 0.375 & 0.390 & 0.375 & 0.393 & \textcolor[HTML]{5CAA82}{-0.04\%} & \textcolor[HTML]{5CAA82}{-0.61\%} & 0.377 & 0.395 & 0.376 & 0.392 & \textcolor{red}{0.39\%} & \textcolor{red}{0.64\%} \\

% & \multicolumn{1}{|c|}{336} & 0.420 & 0.427 & 0.398 & 0.418 & \textcolor{red}{5.16\%} & \textcolor{red}{2.26\%} & 0.414 & 0.424 & 0.405 & 0.423 & \textcolor{red}{2.10\%} & \textcolor{red}{0.26\%} & 0.424 & 0.434 & 0.419 & 0.431 & \textcolor{red}{1.05\%} & \textcolor{red}{0.72\%} \\

% & \multicolumn{1}{|c|}{720} & 0.422 & 0.440 & 0.377 & 0.412 & \textcolor{red}{10.78\%} & \textcolor{red}{6.41\%} & 0.417 & 0.436 & 0.386 & 0.418 & \textcolor{red}{7.43\%} & \textcolor{red}{4.18\%} & 0.433 & 0.448 & 0.422 & 0.443 & \textcolor{red}{2.56\%} & \textcolor{red}{1.14\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.377 & 0.399 & 0.358 & 0.389 & \textcolor{red}{5.02\%} & \textcolor{red}{2.64\%} & 0.374 & 0.397 & 0.363 & 0.393 & \textcolor{red}{2.83\%} & \textcolor{red}{1.18\%} & 0.381 & 0.404 & 0.377 & 0.401 & \textcolor{red}{1.18\%} & \textcolor{red}{0.75\%} \\

% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{Electricity}}
% & \multicolumn{1}{|c|}{96} & 0.197 & 0.274 & 0.140 & 0.234 & \textcolor{red}{29.10\%} & \textcolor{red}{14.48\%} & 0.200 & 0.278 & 0.141 & 0.237 & \textcolor{red}{29.28\%} & \textcolor{red}{14.83\%} & 0.173 & 0.260 & 0.142 & 0.238 & \textcolor{red}{17.50\%} & \textcolor{red}{8.62\%} \\

% & \multicolumn{1}{|c|}{192} & 0.197 & 0.276 & 0.155 & 0.247 & \textcolor{red}{21.57\%} & \textcolor{red}{10.46\%} & 0.199 & 0.280 & 0.214 & 0.295 & \textcolor{red}{21.78\%} & \textcolor{red}{10.82\%} & 0.181 & 0.267 & 0.160 & 0.253 & \textcolor{red}{11.74\%} & \textcolor{red}{5.26\%} \\

% & \multicolumn{1}{|c|}{336} & 0.212 & 0.292 & 0.169 & 0.265 & \textcolor{red}{20.10\%} & \textcolor{red}{9.11\%} & 0.214 & 0.295 & 0.171 & 0.268 & \textcolor{red}{20.18\%} & \textcolor{red}{9.34\%} & 0.196 & 0.283 & 0.175 & 0.271 & \textcolor{red}{11.02\%} & \textcolor{red}{4.21\%} \\

% & \multicolumn{1}{|c|}{720} & 0.253 & 0.324 & 0.198 & 0.290 & \textcolor{red}{21.91\%} & \textcolor{red}{10.43\%} & 0.255 & 0.327 & 0.200 & 0.293 & \textcolor{red}{21.69\%} & \textcolor{red}{10.37\%} & 0.238 & 0.316 & 0.206 & 0.298 & \textcolor{red}{13.43\%} & \textcolor{red}{5.70\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.215 & 0.291 & 0.165 & 0.259 & \textcolor{red}{23.04\%} & \textcolor{red}{11.06\%} & 0.217 & 0.295 & 0.167 & 0.262 & \textcolor{red}{23.09\%} & \textcolor{red}{11.27\%} & 0.197 & 0.282 & 0.171 & 0.265 & \textcolor{red}{13.33\%} & \textcolor{red}{5.90\%} \\

% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}
% & \multicolumn{1}{|c|}{96} & 0.195 & 0.234 & 0.166 & 0.212 & \textcolor{red}{14.91\%} & \textcolor{red}{9.29\%} & 0.194 & 0.235 & 0.167 & 0.213 & \textcolor{red}{14.38\%} & \textcolor{red}{9.16\%} & 0.155 & 0.203 & 0.151 & 0.197 & \textcolor{red}{2.49\%} & \textcolor{red}{3.34\%} \\

% & \multicolumn{1}{|c|}{192} & 0.240 & 0.270 & 0.218 & 0.256 & \textcolor{red}{9.03\%} & \textcolor{red}{5.37\%} & 0.240 & 0.271 & 0.219 & 0.256 & \textcolor{red}{8.92\%} & \textcolor{red}{5.50\%} & 0.202 & 0.247 & 0.200 & 0.244 & \textcolor{red}{1.33\%} & \textcolor{red}{1.37\%} \\

% & \multicolumn{1}{|c|}{336} & 0.291 & 0.306 & 0.272 & 0.294 & \textcolor{red}{6.60\%} & \textcolor{red}{4.02\%} & 0.292 & 0.307 & 0.273 & 0.294 & \textcolor{red}{6.59\%} & \textcolor{red}{4.21\%} & 0.263 & 0.293 & 0.260 & 0.289 & \textcolor{red}{1.23\%} & \textcolor{red}{1.13\%} \\

% & \multicolumn{1}{|c|}{720} & 0.364 & 0.353 & 0.347 & 0.342 & \textcolor{red}{4.81\%} & \textcolor{red}{3.05\%}  & 0.365 & 0.354 & 0.347 & 0.342 & \textcolor{red}{4.85\%} & \textcolor{red}{3.19\%} & 0.341 & 0.343 & 0.338 & 0.338 & \textcolor{red}{0.99\%} & \textcolor{red}{1.34\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.273 & 0.291 & 0.251 & 0.276 & \textcolor{red}{8.02\%} & \textcolor{red}{5.10\%} & 0.273 & 0.292 & 0.251 & 0.277 & \textcolor{red}{7.91\%} & \textcolor{red}{5.20\%} & 0.240 & 0.271 & 0.237 & 0.267 & \textcolor{red}{1.37\%} & \textcolor{red}{1.67\%} \\

% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}
% & \multicolumn{1}{|c|}{96}& 0.645 & 0.383 & 0.459 & 0.293 & \textcolor{red}{28.83\%} & \textcolor{red}{23.45\%} & 0.650 & 0.387 & 0.468 & 0.307 & \textcolor{red}{27.96\%} & \textcolor{red}{20.59\%} & 0.550 & 0.355 & 0.473 & 0.310 & \textcolor{red}{14.09\%} & \textcolor{red}{12.87\%} \\

% & \multicolumn{1}{|c|}{192} & 0.598 & 0.359 & 0.467 & 0.298 & \textcolor{red}{21.83\%} & \textcolor{red}{16.92\%} & 0.602 & 0.363 & 0.480 & 0.315 & \textcolor{red}{20.17\%} & \textcolor{red}{13.28\%} & 0.527 & 0.337 & 0.483 & 0.317 & \textcolor{red}{8.29\%} & \textcolor{red}{5.99\%} \\

% & \multicolumn{1}{|c|}{336} & 0.605 & 0.362 & 0.481 & 0.305 & \textcolor{red}{20.50\%} & \textcolor{red}{15.60\%} & 0.609 & 0.365 & 0.488 & 0.313 & \textcolor{red}{19.82\%} & \textcolor{red}{14.27\%} & 0.537 & 0.342 & 0.503 & 0.328 & \textcolor{red}{6.39\%} & \textcolor{red}{4.12\%} \\

% & \multicolumn{1}{|c|}{720} & 0.643 & 0.381 & 0.512 & 0.320 & \textcolor{red}{20.43\%} & \textcolor{red}{16.11\%} & 0.647 & 0.385 & 0.516 & 0.328 & \textcolor{red}{20.23\%} & \textcolor{red}{14.90\%} & 0.570 & 0.359 & 0.538 & 0.346 & \textcolor{red}{5.59\%} & \textcolor{red}{3.80\%} \\

% \cmidrule(l{10pt}r{10pt}){2-20}
% & \multicolumn{1}{|c|}{Avg} & 0.623 & 0.371 & 0.480 & 0.304 & \textcolor{red}{22.96\%} & \textcolor{red}{18.07\%} & 0.627 & 0.375 & 0.488 & 0.316 & \textcolor{red}{22.12\%} & \textcolor{red}{15.82\%} & 0.546 & 0.348 & 0.499 & 0.325 & \textcolor{red}{8.58\%} & \textcolor{red}{6.72\%} \\

% \midrule
% \multicolumn{2}{c|}{Dataset Avg} & \multicolumn{4}{c|}{} & \textcolor{red}{10.47\%} & \textcolor{red}{6.40\%} & \multicolumn{4}{c|}{} & \textcolor{red}{10.01\%} & \textcolor{red}{5.92\%} & \multicolumn{4}{c|}{} & \textcolor{red}{1.37\%} & \textcolor{red}{1.67\%} \\

% \bottomrule[1pt]
% \setcitestyle{square,numbers,comma}
% \end{tabular}
% }
% % \vspace{-.18cm}
% \end{table*}

\begin{table*}[htpb]
%\setcitestyle{round,numbers,comma}
\caption{Performance gain after combining TimeSter with Linear-based backbones.
The look-back window is $L=96$.
The performance of four prediction lengths $T\in\{96,192,336,720\}$ is reported.
\textit{Avg} indicates the average performance of four prediction lengths.
\textcolor{red}{Red} denotes improved performance and \textcolor[HTML]{5CAA82}{Green} indicates decreasing performance.
\textit{Dataset Avg} denotes the average improvement of a model on all datasets.}
\centering
\label{tab:generalization_full_linear}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{p{0.2cm}c|cc|cc|cc|cc|cc|cc}

\toprule[1pt]

\multicolumn{2}{c|}{Models} & \multicolumn{2}{c}{\makecell{RLinear~\cite{li2023revisiting}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c|}{Promotion} & \multicolumn{2}{c}{\makecell{FITS~\cite{xu2023fits}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c}{Promotion} \\

\cmidrule(l{10pt}r{10pt}){3-4}\cmidrule(l{10pt}r{10pt}){5-6}\cmidrule(l{10pt}r{10pt}){7-8}\cmidrule(l{10pt}r{10pt}){9-10}\cmidrule(l{10pt}r{10pt}){11-12}\cmidrule(l{10pt}r{10pt}){13-14}

\multicolumn{2}{c|}{Metric} & MSE & MAE  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\

\toprule[1pt]
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm1}}
& \multicolumn{1}{|c|}{96} & 0.350 & 0.370 & 0.325 & 0.364 & \textcolor{red}{7.06\%} & \textcolor{red}{1.78\%} & 0.353 & 0.374 & 0.329 & 0.368 & \textcolor{red}{6.77\%} & \textcolor{red}{1.73\%} \\

& \multicolumn{1}{|c|}{192} & 0.389 & 0.390 & 0.365 & 0.381 & \textcolor{red}{6.13\%} & \textcolor{red}{2.26\%} & 0.392 & 0.393 & 0.366 & 0.383 & \textcolor{red}{6.55\%} & \textcolor{red}{2.49\%} \\

& \multicolumn{1}{|c|}{336} & 0.422 & 0.413 & 0.395 & 0.401 & \textcolor{red}{6.43\%} & \textcolor{red}{2.88\%} & 0.425 & 0.415 & 0.397 & 0.402 & \textcolor{red}{6.67\%} & \textcolor{red}{2.98\%} \\

& \multicolumn{1}{|c|}{720} & 0.486 & 0.448 & 0.456 & 0.433 & \textcolor{red}{6.23\%} & \textcolor{red}{3.47\%} & 0.488 & 0.450 & 0.457 & 0.434 & \textcolor{red}{6.42\%} & \textcolor{red}{3.57\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.412 & 0.406 & 0.385 & 0.395 & \textcolor{red}{6.43\%} & \textcolor{red}{2.64\%} & 0.415 & 0.408 & 0.387 & 0.397 & \textcolor{red}{6.59\%} & \textcolor{red}{2.74\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}
& \multicolumn{1}{|c|}{96}& 0.183 & 0.264 & 0.167 & 0.249 & \textcolor{red}{8.48\%} & \textcolor{red}{5.97\%} & 0.183 & 0.266 & 0.168 & 0.249 & \textcolor{red}{8.54\%} & \textcolor{red}{6.25\%} \\

& \multicolumn{1}{|c|}{192} & 0.246 & 0.304 & 0.233 & 0.291 & \textcolor{red}{5.41\%} & \textcolor{red}{4.28\%} & 0.248 & 0.305 & 0.234 & 0.292 & \textcolor{red}{5.45\%} & \textcolor{red}{4.44\%} \\

& \multicolumn{1}{|c|}{336} & 0.307 & 0.342 & 0.295 & 0.331 & \textcolor{red}{4.11\%} & \textcolor{red}{3.24\%} & 0.308 & 0.343 & 0.295 & 0.332 & \textcolor{red}{4.14\%} & \textcolor{red}{3.34\%} \\

& \multicolumn{1}{|c|}{720} & 0.407 & 0.398 & 0.395 & 0.390 & \textcolor{red}{2.96\%} & \textcolor{red}{2.03\%} & 0.408 & 0.398 & 0.396 & 0.390 & \textcolor{red}{2.92\%} & \textcolor{red}{2.25\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.286 & 0.327 & 0.273 & 0.315 & \textcolor{red}{4.68\%} & \textcolor{red}{3.67\%} & 0.286 & 0.328 & 0.273 & 0.316 & \textcolor{red}{4.69\%} & \textcolor{red}{3.85\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh1}}
& \multicolumn{1}{|c|}{96}& 0.389 & 0.395 & 0.378 & 0.391 & \textcolor{red}{2.75\%} & \textcolor{red}{1.00\%} & 0.386 & 0.394 & 0.378 & 0.392 & \textcolor{red}{2.00\%} & \textcolor{red}{0.42\%} \\

& \multicolumn{1}{|c|}{192} & 0.437 & 0.424 & 0.424 & 0.418 & \textcolor{red}{2.95\%} & \textcolor{red}{1.24\%} & 0.438 & 0.424 & 0.424 & 0.418 & \textcolor{red}{3.34\%} & \textcolor{red}{1.48\%} \\

& \multicolumn{1}{|c|}{336} & 0.479 & 0.445 & 0.463 & 0.438 & \textcolor{red}{3.29\%} & \textcolor{red}{1.41\%} & 0.479 & 0.444 & 0.460 & 0.436 & \textcolor{red}{3.89\%} & \textcolor{red}{1.85\%} \\

& \multicolumn{1}{|c|}{720} & 0.480 & 0.469 & 0.464 & 0.456 & \textcolor{red}{3.35\%} & \textcolor{red}{2.75\%} & 0.474 & 0.464 & 0.464 & 0.456 & \textcolor{red}{1.92\%} & \textcolor{red}{1.80\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.446 & 0.433 & 0.432 & 0.426 & \textcolor{red}{3.11\%} & \textcolor{red}{1.64\%} & 0.444 & 0.432 & 0.432 & 0.425 & \textcolor{red}{2.82\%} & \textcolor{red}{1.42\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}
& \multicolumn{1}{|c|}{96}& 0.291 & 0.339 & 0.285 & 0.335 & \textcolor{red}{1.93\%} & \textcolor{red}{1.17\%} & 0.290 & 0.339 & 0.287 & 0.337 & \textcolor{red}{0.97\%} & \textcolor{red}{0.53\%} \\

& \multicolumn{1}{|c|}{192} & 0.376 & 0.390 & 0.373 & 0.390 & \textcolor{red}{0.80\%} & \textcolor{red}{0.07\%} & 0.375 & 0.390 & 0.373 & 0.392 & \textcolor{red}{0.42\%} & \textcolor[HTML]{5CAA82}{-0.49\%} \\

& \multicolumn{1}{|c|}{336} & 0.420 & 0.427 & 0.398 & 0.418 & \textcolor{red}{5.16\%} & \textcolor{red}{2.26\%} & 0.414 & 0.424 & 0.405 & 0.423 & \textcolor{red}{2.10\%} & \textcolor{red}{0.26\%} \\

& \multicolumn{1}{|c|}{720} & 0.422 & 0.440 & 0.377 & 0.412 & \textcolor{red}{10.78\%} & \textcolor{red}{6.41\%} & 0.417 & 0.436 & 0.386 & 0.418 & \textcolor{red}{7.43\%} & \textcolor{red}{4.18\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.377 & 0.399 & 0.358 & 0.389 & \textcolor{red}{5.02\%} & \textcolor{red}{2.64\%} & 0.374 & 0.397 & 0.363 & 0.393 & \textcolor{red}{2.94\%} & \textcolor{red}{1.21\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Electricity}}
& \multicolumn{1}{|c|}{96} & 0.197 & 0.274 & 0.140 & 0.234 & \textcolor{red}{29.10\%} & \textcolor{red}{14.48\%} & 0.200 & 0.278 & 0.141 & 0.237 & \textcolor{red}{29.28\%} & \textcolor{red}{14.83\%} \\

& \multicolumn{1}{|c|}{192} & 0.197 & 0.276 & 0.155 & 0.247 & \textcolor{red}{21.57\%} & \textcolor{red}{10.46\%} & 0.199 & 0.280 & 0.214 & 0.295 & \textcolor{red}{21.78\%} & \textcolor{red}{10.82\%} \\

& \multicolumn{1}{|c|}{336} & 0.212 & 0.292 & 0.169 & 0.265 & \textcolor{red}{20.10\%} & \textcolor{red}{9.11\%} & 0.214 & 0.295 & 0.171 & 0.268 & \textcolor{red}{20.18\%} & \textcolor{red}{9.34\%} \\

& \multicolumn{1}{|c|}{720} & 0.253 & 0.324 & 0.198 & 0.290 & \textcolor{red}{21.91\%} & \textcolor{red}{10.43\%} & 0.255 & 0.327 & 0.200 & 0.293 & \textcolor{red}{21.69\%} & \textcolor{red}{10.37\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.215 & 0.291 & 0.165 & 0.259 & \textcolor{red}{23.04\%} & \textcolor{red}{11.06\%} & 0.217 & 0.295 & 0.167 & 0.262 & \textcolor{red}{23.09\%} & \textcolor{red}{11.27\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}
& \multicolumn{1}{|c|}{96} & 0.195 & 0.234 & 0.166 & 0.212 & \textcolor{red}{14.91\%} & \textcolor{red}{9.29\%} & 0.194 & 0.235 & 0.167 & 0.213 & \textcolor{red}{14.38\%} & \textcolor{red}{9.16\%} \\

& \multicolumn{1}{|c|}{192} & 0.240 & 0.270 & 0.218 & 0.256 & \textcolor{red}{9.03\%} & \textcolor{red}{5.37\%} & 0.240 & 0.271 & 0.219 & 0.256 & \textcolor{red}{8.92\%} & \textcolor{red}{5.50\%} \\

& \multicolumn{1}{|c|}{336} & 0.291 & 0.306 & 0.272 & 0.294 & \textcolor{red}{6.60\%} & \textcolor{red}{4.02\%} & 0.292 & 0.307 & 0.273 & 0.294 & \textcolor{red}{6.59\%} & \textcolor{red}{4.21\%} \\

& \multicolumn{1}{|c|}{720} & 0.364 & 0.353 & 0.347 & 0.342 & \textcolor{red}{4.81\%} & \textcolor{red}{3.05\%}  & 0.365 & 0.354 & 0.347 & 0.342 & \textcolor{red}{4.85\%} & \textcolor{red}{3.19\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.273 & 0.291 & 0.251 & 0.276 & \textcolor{red}{8.02\%} & \textcolor{red}{5.10\%} & 0.273 & 0.292 & 0.251 & 0.277 & \textcolor{red}{7.91\%} & \textcolor{red}{5.20\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}
& \multicolumn{1}{|c|}{96}& 0.645 & 0.383 & 0.459 & 0.293 & \textcolor{red}{28.83\%} & \textcolor{red}{23.45\%} & 0.650 & 0.387 & 0.468 & 0.307 & \textcolor{red}{27.96\%} & \textcolor{red}{20.59\%} \\

& \multicolumn{1}{|c|}{192} & 0.598 & 0.359 & 0.467 & 0.298 & \textcolor{red}{21.83\%} & \textcolor{red}{16.92\%} & 0.602 & 0.363 & 0.480 & 0.315 & \textcolor{red}{20.17\%} & \textcolor{red}{13.28\%} \\

& \multicolumn{1}{|c|}{336} & 0.605 & 0.362 & 0.481 & 0.305 & \textcolor{red}{20.50\%} & \textcolor{red}{15.60\%} & 0.609 & 0.365 & 0.488 & 0.313 & \textcolor{red}{19.82\%} & \textcolor{red}{14.27\%} \\

& \multicolumn{1}{|c|}{720} & 0.643 & 0.381 & 0.512 & 0.320 & \textcolor{red}{20.43\%} & \textcolor{red}{16.11\%} & 0.647 & 0.385 & 0.516 & 0.328 & \textcolor{red}{20.23\%} & \textcolor{red}{14.90\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.623 & 0.371 & 0.480 & 0.304 & \textcolor{red}{22.96\%} & \textcolor{red}{18.07\%} & 0.627 & 0.375 & 0.488 & 0.316 & \textcolor{red}{22.12\%} & \textcolor{red}{15.82\%} \\

\midrule
\multicolumn{2}{c|}{Dataset Avg} & \multicolumn{4}{c|}{} & \textcolor{red}{10.47\%} & \textcolor{red}{6.40\%} & \multicolumn{4}{c|}{} & \textcolor{red}{10.02\%} & \textcolor{red}{5.93\%} \\

\bottomrule[1pt]
%\setcitestyle{square,numbers,comma}
\end{tabular}
}
% \vspace{-.18cm}
\end{table*}

\begin{table*}[htpb]
%\setcitestyle{round,numbers,comma}
\caption{Performance gain after combining TimeSter with Convolution-based backbones.
The look-back window is $L=96$.
The performance of four prediction lengths $T\in\{96,192,336,720\}$ is reported.
\textit{Avg} indicates the average performance of four prediction lengths.
\textcolor{red}{Red} denotes improved performance and \textcolor[HTML]{5CAA82}{Green} indicates decreasing performance.
\textit{Dataset Avg} denotes the average improvement of a model on all datasets.}
\centering
\label{tab:generalization_full_conv}
\resizebox{1\linewidth}{!}{
\begin{tabular}{p{0.2cm}c|cc|cc|cc|cc|cc|cc}

\toprule[1pt]

\multicolumn{2}{c|}{Models} & \multicolumn{2}{c}{\makecell{ModernTCN~\cite{luo2024moderntcn}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c|}{Promotion} & \multicolumn{2}{c}{\makecell{TimesNet~\cite{wu2023timesnet}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c}{Promotion} \\

\cmidrule(l{10pt}r{10pt}){3-4}\cmidrule(l{10pt}r{10pt}){5-6}\cmidrule(l{10pt}r{10pt}){7-8}\cmidrule(l{10pt}r{10pt}){9-10}\cmidrule(l{10pt}r{10pt}){11-12}\cmidrule(l{10pt}r{10pt}){13-14}

\multicolumn{2}{c|}{Metric} & MSE & MAE  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\

\toprule[1pt]
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm1}}
& \multicolumn{1}{|c|}{96} & 0.317 & 0.362 & 0.315 & 0.359 & \textcolor{red}{0.59\%} & \textcolor{red}{0.64\%} & 0.331  & 0.371  & 0.334  & 0.371 & \textcolor[HTML]{5CAA82}{-1.01\%} & \textcolor[HTML]{5CAA82}{-0.05\%} \\

& \multicolumn{1}{|c|}{192} & 0.317 & 0.362 & 0.315 & 0.359 & \textcolor{red}{1.62\%} & \textcolor{red}{0.55\%} & 0.392  & 0.404  & 0.379  & 0.396 & \textcolor{red}{3.40\%} & \textcolor{red}{1.75\%} \\

& \multicolumn{1}{|c|}{336} & 0.403 & 0.412 & 0.399 & 0.411 & \textcolor{red}{1.03\%} & \textcolor{red}{0.06\%} & 0.418  & 0.424  & 0.413  & 0.422 & \textcolor{red}{1.05\%} & \textcolor{red}{0.51\%} \\

& \multicolumn{1}{|c|}{720} & 0.461 & 0.443 & 0.457 & 0.439 & \textcolor{red}{0.94\%} & \textcolor{red}{0.96\%} & 0.490  & 0.460  & 0.480  & 0.456 & \textcolor{red}{1.90\%} & \textcolor{red}{1.05\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.386 & 0.401 & 0.382 & 0.399 & \textcolor{red}{1.05\%} & \textcolor{red}{0.56\%} & 0.408  & 0.415  & 0.402  & 0.411 & \textcolor{red}{1.45\%} & \textcolor{red}{0.84\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}
& \multicolumn{1}{|c|}{96} & 0.173 & 0.255 & 0.169 & 0.252 & \textcolor{red}{1.85\%} & \textcolor{red}{1.14\%} & 0.188  & 0.266  & 0.186  & 0.264 & \textcolor{red}{0.82\%} & \textcolor{red}{0.66\%} \\

& \multicolumn{1}{|c|}{192} & 0.235 & 0.296 & 0.237 & 0.297 & \textcolor[HTML]{5CAA82}{-0.88\%} & \textcolor[HTML]{5CAA82}{-0.20\%} & 0.255  & 0.309  & 0.256  & 0.308 & \textcolor[HTML]{5CAA82}{-0.65\%} & \textcolor{red}{0.43\%} \\

& \multicolumn{1}{|c|}{336} & 0.308 & 0.344 & 0.299 & 0.336 & \textcolor{red}{2.80\%} & \textcolor{red}{2.20\%} & 0.319  & 0.347  & 0.312  & 0.343 & \textcolor{red}{2.23\%} & \textcolor{red}{1.12\%} \\

& \multicolumn{1}{|c|}{720} & 0.398 & 0.394 & 0.395 & 0.392 & \textcolor{red}{0.61\%} & \textcolor{red}{0.34\%} & 0.419  & 0.406  & 0.413  & 0.401 & \textcolor{red}{1.39\%} & \textcolor{red}{1.05\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.278 & 0.322 & 0.275 & 0.319 & \textcolor{red}{1.09\%} & \textcolor{red}{0.87\%} & 0.295  & 0.332  & 0.292  & 0.329 & \textcolor{red}{1.08\%} & \textcolor{red}{0.85\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh1}}
& \multicolumn{1}{|c|}{96} & 0.386 & 0.394 & 0.385 & 0.394 & \textcolor{red}{0.09\%} & \textcolor{red}{0.05\%} & 0.399  & 0.419  & 0.401  & 0.420 & \textcolor[HTML]{5CAA82}{-0.48\%} & \textcolor[HTML]{5CAA82}{-0.16\%} \\

& \multicolumn{1}{|c|}{192} & 0.436 & 0.423 & 0.436 & 0.423 & \textcolor{red}{0.01\%} & \textcolor{red}{0.01\%} & 0.453  & 0.449  & 0.451  & 0.450 & \textcolor{red}{0.51\%} & \textcolor[HTML]{5CAA82}{-0.27\%} \\

& \multicolumn{1}{|c|}{336} & 0.479 & 0.445 & 0.477 & 0.444 & \textcolor{red}{0.37\%} & \textcolor{red}{0.22\%} & 0.507  & 0.480  & 0.502  & 0.477 & \textcolor{red}{0.88\%} & \textcolor{red}{0.57\%} \\

& \multicolumn{1}{|c|}{720} & 0.481 & 0.469 & 0.479 & 0.466 & \textcolor{red}{0.40\%} & \textcolor{red}{0.54\%} & 0.532  & 0.502  & 0.505  & 0.490 & \textcolor{red}{4.99\%} & \textcolor{red}{2.42\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.445 & 0.432 & 0.444 & 0.432 & \textcolor{red}{0.23\%} & \textcolor{red}{0.22\%} & 0.473  & 0.463  & 0.465  & 0.459 & \textcolor{red}{1.66\%} & \textcolor{red}{0.70\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}
& \multicolumn{1}{|c|}{96} & 0.292 & 0.340 & 0.290 & 0.339 & \textcolor{red}{0.35\%} & \textcolor{red}{0.40\%} & 0.322  & 0.363  & 0.324  & 0.367 & \textcolor[HTML]{5CAA82}{-0.57\%} & \textcolor[HTML]{5CAA82}{-0.91\%} \\

& \multicolumn{1}{|c|}{192} & 0.377 & 0.395 & 0.376 & 0.392 & \textcolor{red}{0.39\%} & \textcolor{red}{0.64\%} & 0.404  & 0.413  & 0.399  & 0.411 & \textcolor{red}{1.18\%} & \textcolor{red}{0.53\%} \\

& \multicolumn{1}{|c|}{336} & 0.424 & 0.434 & 0.419 & 0.431 & \textcolor{red}{1.05\%} & \textcolor{red}{0.72\%} & 0.448  & 0.449  & 0.438  & 0.443 & \textcolor{red}{2.26\%} & \textcolor{red}{1.42\%} \\

& \multicolumn{1}{|c|}{720} & 0.433 & 0.448 & 0.422 & 0.443 & \textcolor{red}{2.56\%} & \textcolor{red}{1.14\%} & 0.453  & 0.460  & 0.434  & 0.450 & \textcolor{red}{4.27\%} & \textcolor{red}{2.22\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.381 & 0.404 & 0.377 & 0.401 & \textcolor{red}{1.18\%} & \textcolor{red}{0.75\%} & 0.407  & 0.421  & 0.399  & 0.417 & \textcolor{red}{1.99\%} & \textcolor{red}{0.92\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Electricity}}
& \multicolumn{1}{|c|}{96} & 0.173 & 0.260 & 0.142 & 0.238 & \textcolor{red}{17.50\%} & \textcolor{red}{8.62\%} & 0.167  & 0.271  & 0.166  & 0.269 & \textcolor{red}{0.80\%} & \textcolor{red}{0.56\%} \\

& \multicolumn{1}{|c|}{192} & 0.181 & 0.267 & 0.160 & 0.253 & \textcolor{red}{11.74\%} & \textcolor{red}{5.26\%} & 0.186  & 0.288  & 0.184  & 0.286 & \textcolor{red}{1.15\%} & \textcolor{red}{0.69\%} \\

& \multicolumn{1}{|c|}{336} & 0.196 & 0.283 & 0.175 & 0.271 & \textcolor{red}{11.02\%} & \textcolor{red}{4.21\%} & 0.203  & 0.303  & 0.194  & 0.295 & \textcolor{red}{4.58\%} & \textcolor{red}{2.63\%} \\

& \multicolumn{1}{|c|}{720} & 0.238 & 0.316 & 0.206 & 0.298 & \textcolor{red}{13.43\%} & \textcolor{red}{5.70\%} & 0.225  & 0.320  & 0.228  & 0.322 & \textcolor[HTML]{5CAA82}{-1.57\%} & \textcolor[HTML]{5CAA82}{-0.61\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.197 & 0.282 & 0.171 & 0.265 & \textcolor{red}{13.33\%} & \textcolor{red}{5.90\%} & 0.195  & 0.295  & 0.193  & 0.293 & \textcolor{red}{1.19\%} & \textcolor{red}{0.80\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}
& \multicolumn{1}{|c|}{96} & 0.155 & 0.203 & 0.151 & 0.197 & \textcolor{red}{2.49\%} & \textcolor{red}{3.34\%} & 0.172  & 0.222  & 0.166  & 0.216 & \textcolor{red}{3.50\%} & \textcolor{red}{2.88\%} \\

& \multicolumn{1}{|c|}{192} & 0.202 & 0.247 & 0.200 & 0.244 & \textcolor{red}{1.33\%} & \textcolor{red}{1.37\%} & 0.229  & 0.268  & 0.216  & 0.259 & \textcolor{red}{5.48\%} & \textcolor{red}{3.66\%} \\

& \multicolumn{1}{|c|}{336} & 0.263 & 0.293 & 0.260 & 0.289 & \textcolor{red}{1.23\%} & \textcolor{red}{1.13\%} & 0.284  & 0.305  & 0.274  & 0.299 & \textcolor{red}{3.65\%} & \textcolor{red}{1.87\%} \\

& \multicolumn{1}{|c|}{720} & 0.341 & 0.343 & 0.338 & 0.338 & \textcolor{red}{0.99\%} & \textcolor{red}{1.34\%} & 0.357  & 0.354  & 0.351  & 0.349 & \textcolor{red}{1.67\%} & \textcolor{red}{1.29\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.240 & 0.271 & 0.237 & 0.267 & \textcolor{red}{1.37\%} & \textcolor{red}{1.67\%} & 0.261  & 0.287  & 0.252  & 0.281 & \textcolor{red}{3.35\%} & \textcolor{red}{2.30\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}
& \multicolumn{1}{|c|}{96} & 0.523 & 0.350 & 0.465 & 0.304 & \textcolor{red}{11.07\%} & \textcolor{red}{13.15\%} & 0.590  & 0.315  & 0.588  & 0.314 & \textcolor{red}{0.21\%} & \textcolor{red}{0.25\%} \\

& \multicolumn{1}{|c|}{192} & 0.543 & 0.366 & 0.475 & 0.312 & \textcolor{red}{12.50\%} & \textcolor{red}{14.75\%} & 0.617  & 0.329  & 0.612  & 0.326 & \textcolor{red}{0.78\%} & \textcolor{red}{0.85\%} \\

& \multicolumn{1}{|c|}{336} & 0.544 & 0.366 & 0.494 & 0.323 & \textcolor{red}{9.17\%} & \textcolor{red}{11.75\%} & 0.636  & 0.337  & 0.630  & 0.334 & \textcolor{red}{0.98\%} & \textcolor{red}{0.73\%} \\

& \multicolumn{1}{|c|}{720} & 0.590 & 0.395 & 0.532 & 0.344 & \textcolor{red}{9.85\%} & \textcolor{red}{12.83\%} & 0.668  & 0.353  & 0.665  & 0.349 & \textcolor{red}{0.43\%} & \textcolor{red}{1.06\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.550 & 0.369 & 0.499 & 0.325 & \textcolor{red}{10.63\%} & \textcolor{red}{13.12\%} & 0.628  & 0.333  & 0.624  & 0.331 & \textcolor{red}{0.60\%} & \textcolor{red}{0.73\%} \\

\midrule
\multicolumn{2}{c|}{Dataset Avg} & \multicolumn{4}{c|}{} & \textcolor{red}{4.13\%} & \textcolor{red}{3.30\%} & \multicolumn{4}{c|}{} & \textcolor{red}{1.62\%} & \textcolor{red}{1.02\%} \\

\bottomrule[1pt]
%\setcitestyle{square,numbers,comma}
\end{tabular}
}
% \vspace{-.18cm}
\end{table*}

\begin{table*}[htpb]
%\setcitestyle{round,numbers,comma}
\caption{Performance gain after combining TimeSter with Transformer-based backbones.
The look-back window is $L=96$.
The performance of four prediction lengths $T\in\{96,192,336,720\}$ is reported.
\textit{Avg} indicates the average performance of four prediction lengths.
\textcolor{red}{Red} denotes improved performance and \textcolor[HTML]{5CAA82}{Green} indicates decreasing performance.
\textit{Dataset Avg} denotes the average improvement of a model on all datasets.}
\centering
\label{tab:generalization_full_trans}
\resizebox{1\linewidth}{!}{
\begin{tabular}{p{0.2cm}c|cc|cc|cc|cc|cc|cc}

\toprule[1pt]

\multicolumn{2}{c|}{Models} & \multicolumn{2}{c}{\makecell{iTransformer~\cite{liu2024itransformer}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c|}{Promotion} & \multicolumn{2}{c}{\makecell{PatchTST~\cite{Yuqietal-2023-PatchTST}}} & \multicolumn{2}{c}{w / TimeSter} & \multicolumn{2}{c}{Promotion} \\

\cmidrule(l{10pt}r{10pt}){3-4}\cmidrule(l{10pt}r{10pt}){5-6}\cmidrule(l{10pt}r{10pt}){7-8}\cmidrule(l{10pt}r{10pt}){9-10}\cmidrule(l{10pt}r{10pt}){11-12}\cmidrule(l{10pt}r{10pt}){13-14}

\multicolumn{2}{c|}{Metric} & MSE & MAE  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\

\toprule[1pt]
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm1}}
& \multicolumn{1}{|c|}{96} & 0.341  & 0.376  & 0.325  & 0.369  & \textcolor{red}{4.60\%} & \textcolor{red}{1.85\%} & 0.325  & 0.364  & 0.316  & 0.363  & \textcolor{red}{3.00\%} & \textcolor{red}{0.36\%} \\

& \multicolumn{1}{|c|}{192} & 0.382  & 0.395  & 0.367  & 0.390  & \textcolor{red}{3.90\%} & \textcolor{red}{1.47\%} & 0.368  & 0.388  & 0.362  & 0.390  & \textcolor{red}{1.67\%} & \textcolor[HTML]{5CAA82}{-0.67\%} \\

& \multicolumn{1}{|c|}{336} & 0.419  & 0.419  & 0.402  & 0.411  & \textcolor{red}{4.07\%} & \textcolor{red}{1.78\%} & 0.396  & 0.405  & 0.387  & 0.405  & \textcolor{red}{2.42\%} & \textcolor[HTML]{5CAA82}{-0.03\%} \\

& \multicolumn{1}{|c|}{720} & 0.490  & 0.458  & 0.469  & 0.448  & \textcolor{red}{4.39\%} & \textcolor{red}{2.31\%} & 0.459  & 0.444  & 0.451  & 0.446  & \textcolor{red}{1.72\%} & \textcolor[HTML]{5CAA82}{-0.34\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.408  & 0.412  & 0.391  & 0.404  & \textcolor{red}{4.24\%} & \textcolor{red}{1.87\%} & 0.387  & 0.400  & 0.379  & 0.401  & \textcolor{red}{2.15\%} & \textcolor[HTML]{5CAA82}{-0.18\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}
& \multicolumn{1}{|c|}{96} & 0.185  & 0.270  & 0.174  & 0.258  & \textcolor{red}{5.80\%} & \textcolor{red}{4.64\%} & 0.179  & 0.260  & 0.170  & 0.254  & \textcolor{red}{4.96\%} & \textcolor{red}{2.28\%} \\

& \multicolumn{1}{|c|}{192} & 0.252  & 0.312  & 0.243  & 0.303  & \textcolor{red}{3.55\%} & \textcolor{red}{3.06\%} & 0.242  & 0.302  & 0.241  & 0.302  & \textcolor{red}{0.45\%} & \textcolor{red}{0.00\%} \\

& \multicolumn{1}{|c|}{336} & 0.314  & 0.351  & 0.302  & 0.340  & \textcolor{red}{3.79\%} & \textcolor{red}{3.07\%} & 0.306  & 0.345  & 0.298  & 0.340  & \textcolor{red}{2.50\%} & \textcolor{red}{1.43\%} \\

& \multicolumn{1}{|c|}{720} & 0.412  & 0.406  & 0.403  & 0.398  & \textcolor{red}{2.23\%} & \textcolor{red}{2.00\%} & 0.406  & 0.402  & 0.401  & 0.400  & \textcolor{red}{1.30\%} & \textcolor{red}{0.39\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.291  & 0.335  & 0.280  & 0.325  & \textcolor{red}{3.50\%} & \textcolor{red}{3.06\%} & 0.283  & 0.327  & 0.278  & 0.324  & \textcolor{red}{2.02\%} & \textcolor{red}{0.95\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh1}}
& \multicolumn{1}{|c|}{96} & 0.385  & 0.404  & 0.383  & 0.402  & \textcolor{red}{0.67\%} & \textcolor{red}{0.49\%} & 0.377  & 0.396  & 0.377  & 0.396  & \textcolor{red}{0.03\%} & \textcolor{red}{0.10\%} \\

& \multicolumn{1}{|c|}{192} & 0.443  & 0.437  & 0.431  & 0.429  & \textcolor{red}{2.65\%} & \textcolor{red}{1.83\%} & 0.425  & 0.427  & 0.422  & 0.425  & \textcolor{red}{0.74\%} & \textcolor{red}{0.38\%} \\

& \multicolumn{1}{|c|}{336} & 0.487  & 0.458  & 0.473  & 0.449  & \textcolor{red}{2.94\%} & \textcolor{red}{1.98\%} & 0.461  & 0.447  & 0.459  & 0.446  & \textcolor{red}{0.52\%} & \textcolor{red}{0.31\%} \\

& \multicolumn{1}{|c|}{720} & 0.517  & 0.497  & 0.470  & 0.470  & \textcolor{red}{9.07\%} & \textcolor{red}{5.61\%} & 0.518  & 0.493  & 0.496  & 0.489  & \textcolor{red}{4.29\%} & \textcolor{red}{0.89\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.458  & 0.449  & 0.439  & 0.437  & \textcolor{red}{4.12\%} & \textcolor{red}{2.61\%} & 0.445  & 0.441  & 0.438  & 0.439  & \textcolor{red}{1.57\%} & \textcolor{red}{0.44\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTh2}}
& \multicolumn{1}{|c|}{96} & 0.299  & 0.350  & 0.295  & 0.346  & \textcolor{red}{1.44\%} & \textcolor{red}{1.04\%} & 0.294  & 0.343  & 0.290  & 0.340  & \textcolor{red}{1.51\%} & \textcolor{red}{0.73\%} \\

& \multicolumn{1}{|c|}{192} & 0.380  & 0.399  & 0.377  & 0.398  & \textcolor{red}{0.77\%} & \textcolor{red}{0.17\%} & 0.377  & 0.398  & 0.364  & 0.389  & \textcolor{red}{3.41\%} & \textcolor{red}{2.14\%} \\

& \multicolumn{1}{|c|}{336} & 0.423  & 0.432  & 0.419  & 0.431  & \textcolor{red}{0.93\%} & \textcolor{red}{0.37\%} & 0.414  & 0.426  & 0.408  & 0.426  & \textcolor{red}{1.39\%} & \textcolor{red}{0.01\%} \\

& \multicolumn{1}{|c|}{720} & 0.429  & 0.446  & 0.419  & 0.441  & \textcolor{red}{2.22\%} & \textcolor{red}{1.18\%} & 0.426  & 0.445  & 0.421  & 0.441  & \textcolor{red}{1.15\%} & \textcolor{red}{0.89\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.383  & 0.407  & 0.378  & 0.404  & \textcolor{red}{1.35\%} & \textcolor{red}{0.69\%} & 0.378  & 0.403  & 0.371  & 0.399  & \textcolor{red}{1.85\%} & \textcolor{red}{0.93\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Electricity}}
& \multicolumn{1}{|c|}{96} & 0.148  & 0.240  & 0.134  & 0.232  & \textcolor{red}{9.49\%} & \textcolor{red}{3.56\%} & 0.165  & 0.256  & 0.142  & 0.240  & \textcolor{red}{13.92\%} & \textcolor{red}{5.95\%} \\

& \multicolumn{1}{|c|}{192} & 0.165  & 0.256  & 0.152  & 0.248  & \textcolor{red}{7.68\%} & \textcolor{red}{3.19\%} & 0.174  & 0.265  & 0.160  & 0.258  & \textcolor{red}{8.33\%} & \textcolor{red}{2.69\%} \\

& \multicolumn{1}{|c|}{336} & 0.178  & 0.270  & 0.167  & 0.267  & \textcolor{red}{6.34\%} & \textcolor{red}{1.45\%} & 0.191  & 0.282  & 0.173  & 0.273  & \textcolor{red}{9.50\%} & \textcolor{red}{3.13\%} \\

& \multicolumn{1}{|c|}{720} & 0.221  & 0.308  & 0.195  & 0.292  & \textcolor{red}{11.67\%} & \textcolor{red}{5.04\%} & 0.232  & 0.316  & 0.202  & 0.300  & \textcolor{red}{12.84\%} & \textcolor{red}{5.17\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.178  & 0.269  & 0.162  & 0.260  & \textcolor{red}{8.96\%} & \textcolor{red}{3.36\%} & 0.191  & 0.280  & 0.169  & 0.268  & \textcolor{red}{11.20\%} & \textcolor{red}{4.25\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}
& \multicolumn{1}{|c|}{96} & 0.174  & 0.213  & 0.160  & 0.205  & \textcolor{red}{8.18\%} & \textcolor{red}{4.09\%} & 0.173  & 0.214  & 0.157  & 0.205  & \textcolor{red}{9.49\%} & \textcolor{red}{4.27\%} \\

& \multicolumn{1}{|c|}{192} & 0.224  & 0.257  & 0.214  & 0.252  & \textcolor{red}{4.66\%} & \textcolor{red}{1.99\%} & 0.219  & 0.255  & 0.208  & 0.250  & \textcolor{red}{5.12\%} & \textcolor{red}{2.31\%} \\

& \multicolumn{1}{|c|}{336} & 0.281  & 0.299  & 0.271  & 0.294  & \textcolor{red}{3.69\%} & \textcolor{red}{1.69\%} & 0.277  & 0.297  & 0.265  & 0.290  & \textcolor{red}{4.58\%} & \textcolor{red}{2.22\%} \\

& \multicolumn{1}{|c|}{720} & 0.359  & 0.351  & 0.349  & 0.346  & \textcolor{red}{2.77\%} & \textcolor{red}{1.47\%} & 0.354  & 0.347  & 0.342  & 0.341  & \textcolor{red}{3.30\%} & \textcolor{red}{1.54\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.260  & 0.280  & 0.249  & 0.274  & \textcolor{red}{4.33\%} & \textcolor{red}{2.15\%} & 0.256  & 0.278  & 0.243  & 0.272  & \textcolor{red}{5.08\%} & \textcolor{red}{2.42\%} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}
& \multicolumn{1}{|c|}{96} & 0.393  & 0.269  & 0.392  & 0.267  & \textcolor{red}{0.43\%} & \textcolor{red}{0.40\%} & 0.437  & 0.280  & 0.416  & 0.279  & \textcolor{red}{4.79\%} & \textcolor{red}{0.08\%} \\

& \multicolumn{1}{|c|}{192} & 0.413  & 0.277  & 0.414  & 0.277  & \textcolor[HTML]{5CAA82}{-0.34\%} & \textcolor{red}{0.13\%} & 0.448  & 0.284  & 0.429  & 0.284  & \textcolor{red}{4.24\%} & \textcolor[HTML]{5CAA82}{-0.23\%} \\

& \multicolumn{1}{|c|}{336} & 0.424  & 0.283  & 0.427  & 0.283  & \textcolor[HTML]{5CAA82}{-0.66\%} & \textcolor{red}{0.03\%} & 0.463  & 0.292  & 0.444  & 0.291  & \textcolor{red}{4.15\%} & \textcolor{red}{0.05\%} \\

& \multicolumn{1}{|c|}{720} & 0.459  & 0.301  & 0.455  & 0.297  & \textcolor{red}{1.03\%} & \textcolor{red}{1.30\%} & 0.497  & 0.310  & 0.477  & 0.309  & \textcolor{red}{3.91\%} & \textcolor{red}{0.17\%} \\

\cmidrule(l{10pt}r{10pt}){2-14}
& \multicolumn{1}{|c|}{Avg} & 0.422  & 0.282  & 0.422  & 0.281  & \textcolor{red}{0.13\%} & \textcolor{red}{0.48\%} & 0.461  & 0.291  & 0.442  & 0.291  & \textcolor{red}{4.26\%} & \textcolor{red}{0.02\%} \\

\midrule
\multicolumn{2}{c|}{Dataset Avg} & \multicolumn{4}{c|}{} & \textcolor{red}{3.81\%} & \textcolor{red}{2.03\%} & \multicolumn{4}{c|}{} & \textcolor{red}{4.02\%} & \textcolor{red}{1.26\%} \\

\bottomrule[1pt]
%\setcitestyle{square,numbers,comma}
\end{tabular}
}
% \vspace{-.18cm}
\end{table*}

==> table/hyper.tex <==
\begin{table*}[t]
\caption{Learning rate and batch size for each dataset. The column with more than one value indicates we choose different values in different prediction lengths.}
\centering
\label{tab:hyper}
\renewcommand{\arraystretch}{1.0}
\begin{tabularx}{\textwidth}{c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}

\toprule[1pt]
\multicolumn{1}{c|}{{Dataset}} & ETTm1  & ETTm2 & ETTh1 & ETTh2 & Electricity & Weather & Traffic \\

\toprule[1pt]
Learning rate & 1e-2 & 1e-2 & 1e-2 & 1e-2 & 1e-2 & 5e-3 & 5e-3 \\
Batch size & 128 & 64 & 64 \& 128 & 64 \& 128 & 16 & 128 & 16 \\

\bottomrule[1pt]
\end{tabularx}

% \vspace{-.18cm}
\end{table*}


==> table/notation.tex <==
\begin{table}[h]
	\caption{Notation des SCLSP-RM\textsuperscript{gen} Modells nach Sahling et all.(2016)}
%\resizebox{1.0\linewidth}{!}{
    \begin{tabularx}{\linewidth}{p{0.09\textwidth}X}
		\toprule	
		\underline{\textbf{\emph{Indices}}} \\
		$L$ & length of historical window  \\ 
		$T$ & length of prediction window \\
        $V$ & number of time series variables \\
        $r$ & number of time-related features \\
		\underline{\textbf{\emph{Parameters}}} \\  
		$\mathbf{X}\in\mathbb{R}^{L\times V}$ & multivariate historical observations \\
		%$\mathbf{X}_{\mathbf{U}}\in\mathbb{R}^{L\times V}$ & multivariate historical time-related observations \\
		$\mathbf{Y}\in\mathbb{R}^{T\times V}$ & multivariate future observations \\
		%$\mathbf{Y}_{\mathbf{U}}\in\mathbb{R}^{U\times V}$ & multivariate future time-related observations \\
		$\mathbf{U}\in\mathbb{R}^{L\times r}$ & historical time-related features \\
		$\mathbf{P}\in\mathbb{R}^{T\times r}$ & future time-related features \\
		\underline{\textbf{\emph{Random variables}}} \\ 
		$\mathbf{W}$  & learnable weights \\
		$\mathbf{b}$  & learnable bias \\
		$f(\cdot),g(\cdot)$  & linear projectors \\
		\bottomrule
    \end{tabularx}
%}
\end{table}

